Coherent suppression of backscattering in optical microresonators

As light propagates along a waveguide, a fraction of the field can be reflected by Rayleigh scatterers. In high-quality-factor whispering-gallery-mode microresonators, this intrinsic backscattering is primarily caused by either surface or bulk material imperfections. For several types of microresonator-based experiments and applications, minimal backscattering in the cavity is of critical importance, and thus, the ability to suppress backscattering is essential. We demonstrate that the introduction of an additional scatterer into the near field of a high-quality-factor microresonator can coherently suppress the amount of backscattering in the microresonator by more than 30 dB. The method relies on controlling the scatterer position such that the intrinsic and scatterer-induced backpropagating fields destructively interfere. This technique is useful in microresonator applications where backscattering is currently limiting the performance of devices, such as ring-laser gyroscopes and dual frequency combs, which both suffer from injection locking. Moreover, these findings are of interest for integrated photonic circuits in which back reflections could negatively impact the stability of laser sources or other components.

==> 0 Arxiv versions/addendum.tex <==
\subsubsection*{Acknowledgements} This work has been supported by the National Physical Laboratory Strategic Research Programme and the European Research Council (CounterLight, 756966), Marie Sk\l odowska-Curie Actions (MSCA) (CoLiDR, 748519) and UK Research and Innovation (MR/S032924/1). A.\O.S. is supported by an Aker Scholarship and the Engineering and Physical Sciences Research Council (EPSRC) via the Quantum Systems Engineering programme at Imperial College London. J.M.S. acknowledges funding via a Royal Society of Engineering fellowship. L.D.B. and M.T.M.W. are supported by the EPSRC through the Centre for Doctoral Training in Applied Photonics. S.Z. acknowledges funding via an MSCA fellowship (GA-2015-713694).

\newpage
\subsubsection*{Author contributions} A.\O.S. and P.D'H. conceived the experiments. A.\O.S., L.D.B., J.M.S., S.Z. and M.T.M.W. designed and constructed the experiments. 
A.\O.S. performed the experiments and analysed the results with J.M.S. All authors discussed the project, its results, and contributed to the manuscript.

\subsubsection*{Data availability} The data that supports this Article is available from the corresponding author upon reasonable request.

\subsubsection*{Competing interests} The authors declare that they have no competing financial interests.

\subsubsection*{Additional information} Correspondence and requests for materials should be addressed to P.D'H.~(email: pascal.delhaye@mpl.mpg.de).


==> 0 Arxiv versions/authors.tex <==
\author{Andreas~\O.~Svela}
\affiliation{National Physical Laboratory, Teddington, TW11 0LW, UK}
\affiliation{Blackett Laboratory, Imperial College London, SW7 2AZ, UK}
\affiliation{Clarendon Laboratory, University of Oxford, OX1 3PU, UK}

\author{Jonathan~M.~Silver}
\affiliation{National Physical Laboratory, Teddington, TW11 0LW, UK}
\affiliation{City, University of London, EC1V 0HB, UK}

\author{Leonardo~Del~Bino}
\affiliation{National Physical Laboratory, Teddington, TW11 0LW, UK}
\affiliation{Heriot-Watt University, Edinburgh, Scotland, EH14 4AS, UK}
\affiliation{Max Planck Institute for the Science of Light, Staudtsta{\ss}e 2, 91058 Erlangen, Germany}

\author{Shuangyou~Zhang}
\affiliation{National Physical Laboratory, Teddington, TW11 0LW, UK}
\affiliation{Max Planck Institute for the Science of Light, Staudtsta{\ss}e 2, 91058 Erlangen, Germany}

\author{Michael~T.~M.~Woodley}
\affiliation{National Physical Laboratory, Teddington, TW11 0LW, UK}
\affiliation{Blackett Laboratory, Imperial College London, SW7 2AZ, UK}
\affiliation{Heriot-Watt University, Edinburgh, Scotland, EH14 4AS, UK}

\author{Michael~R.~Vanner}
\affiliation{Blackett Laboratory, Imperial College London, SW7 2AZ, UK}
\affiliation{Clarendon Laboratory, University of Oxford, OX1 3PU, UK}

\author{Pascal~Del'Haye}
\thanks{pascal.delhaye@mpl.mpg.de}
\affiliation{National Physical Laboratory, Teddington, TW11 0LW, UK}
\affiliation{Max Planck Institute for the Science of Light, Staudtsta{\ss}e 2, 91058 Erlangen, Germany}
\affiliation{Friedrich Alexander University Erlangen-Nuremberg, 91058 Erlangen, Germany}

==> 0 Arxiv versions/methods.tex <==
% METHODS ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ %
\section{Materials and methods}

\subsection{Resonator and tapered fibre fabrication.}
The rod resonators were machined using a \SI{100}{\watt} CO$_2$ laser, milling commercially available 3-\si{\milli\metre}-diameter silica glass rods. The procedure follows that of Del'Haye~\textit{et.~al.}\citeL{DelHaye2013}, but to reach the highest Q-factor of $\num{e9}$, the resonator is fabricated in a nitrogen atmosphere, seeking to avoid the formation of near-IR-absorbing \ce{OH} groups. The rod is fixed to a spindle motor and the glass is evaporated with the focused laser beam. First, the low (high) $Q$ rod was milled down to a 2.7-\si{\milli\metre}-diameter (1.7-\si{\milli\metre}-diameter) cylindrical shape, then the resonator was created by making two ring cuts separated by $\sim\SI{125}{\micro\metre}$ ($\sim\SI{240}{\micro\metre}$).

The tapered fibre was made from a stripped 125-\si{\micro\metre}-diameter standard single-mode silica optical fibre. The fibre was clamped to stepper motor stages, with a hydrogen flame placed under the fibre to heat it while simultaneously pulling symmetrically from both sides.


\subsection{Tungsten tip fabrication.}
The fabrication of the tungsten tip was based on methods used in scanning tunnelling electron microscopy and atomic force microscopy tip fabrication\citeL{Ibe1990,Hagedorn2011}. The process relies surface tension to form a meniscus of solution around a piece of tungsten wire and on the aqueous electrochemical reaction
\begin{equation*}
	\ce{W(solid) + 2 OH^- + 2 H2O -> WO4^2- + 3 H2(gas)}
\end{equation*}
etching the solid tungsten (\ce{W}) anode through oxidation. When the minimum potential difference (\SI{1.43}{\volt}) is overcome, the etching rate varies along the wire due to a hydroxide concentration gradient: the etching rate is slower on the top of the meniscus as the `hydroxide supply' is lower in the meniscus above the horizontal surface. This causes a tip shape to form. Further down, the wire is protected as the tungstate (\ce{WO4^2-}) ions fall along the sides of the wire, forming an increasingly dense laminar layer, protecting the lower end of the tip from being etched. When the diameter at the meniscus is decreased sufficiently, gravity will break off the lower part of the wire.

Temper-annealed, 250-\si{\micro\metre}-diameter, \SI{99.95}{\percent} purity polycrystalline tungsten wire was used in the fabrication. The electrolyte was made by dissolving potassium hydroxide (\ce{KOH}) in deionised water, making a \SI{7.5}{\mol\per\liter} concentration aqueous solution. The second electrode used was tinned copper electrical wire of diameter \SI{0.3}{\milli\metre}. The tungsten wire was pre-etched for five seconds at \SI{4}{\volt} to reduce the surface roughness. After pre-etching, the wire was lifted $\sim\SI{1}{\milli\metre}$ before continuing the etching process at \SI{4}{\volt} until the lower part fell off. The total etching time was approximately two minutes.


\subsection{Experimental setup.}
A fibre-coupled external cavity diode laser at \SI{1.55}{\micro\metre}, connected to an erbium-doped fibre amplifier, was used as the light source in the experiments. To obtain spectral measurements of the microresonator mode, the frequency of the laser source was scanned by current modulation with a triangular wave signal at \SI{1007}{\hertz} (\cref{fig:firstmment}) and \SI{20}{\hertz} (\cref{fig:secondmment}). As the light was subsequently fed into an amplifier operating in saturation, the optical power was kept constant. A polarisation controller was used for optimising coupling to a resonator mode, and a circulator to separate out the backward-propagating light in the tapered fibre for detection. The tapered fibre was mounted on a manual piezo stage to control the coupling to the resonator. Amplified photodetectors and an oscilloscope were used for simultaneously monitoring the transmission and backscattered light.

The tungsten tip was fixed to a polylactic acid (PLA) plastic mount, sitting on a three-axis piezo positioner. The tip position was raster-scanned over a $\SI{1}{\micro\metre}\times\SI{1.5}{\micro\metre}$ area in the resonator plane, and spectra for backscattering and transmission were obtained for each \SI{50}{\nano\metre} (\cref{fig:firstmment}) or \SI{25}{\nano\metre} (\cref{fig:secondmment}) step. The tip-positioner and oscilloscope were simultaneously computer-controlled, allowing a capture time of a few minutes for each of the two measurements reported.


\subsection{Data analysis.}
Least squares fitting procedures were applied to the spectra obtained in the measurement, determining the pump transmission half-linewidth $\gamma$ and amplitude $A_\pump$, and backscattering amplitude $A_\bs$ of the cavity for each position in the measurement. No spectrally resolvable mode splitting was observed.

For the pump resonance, a normal Lorentzian dip from a background $B$ is used, $B-A_\pump/(1+\delta^2/\gamma^2)$, where the detuning with respect to the resonance angular frequency $\omega_0$ is $\delta = \omega - \omega_0$. However, the spectral shape for the backscattering is distorted as it is effectively pumped by a Lorentzian (the pump resonance), resulting in a lineshape $A_\bs/(1+\delta^2/\gamma^2)^2$ in the limit of small backscattering (see Supplementary information for the derivation).

Subsequent to fitting the individual measurements, the grid data of linewidth and backscattering amplitude measurements were fitted. The functions used for the grid data fitting are expressed in a rotated (cartesian) coordinate system $(r,\phi)$ at an angle $\beta$ to the measurement coordinate system $(x,y)$, where the coordinate transformation is given by
\begin{equation*}
	\begin{pmatrix}
		r\\
		\phi
	\end{pmatrix} = 
	\begin{pmatrix}
		\cos\beta & -\sin\beta \\
		\sin\beta &  \cos\beta
	\end{pmatrix}
	\begin{pmatrix}
		x\\
		y
	\end{pmatrix}.
\end{equation*}
In this coordinate system, the $r$ axis is normal to the resonator surface, and $\phi$ can be approximated as the azimuthal position over a short distance compared to the resonator's radius of curvature. The rotation angle $\beta$ was determined as one of the free parameters of the linewidth grid fit, where the linewidth function expressed in the $(r,\phi)$ coordinate system is
\begin{equation*}
	\gamma\,(r,\phi) = \gamma_0 + 
		\begin{cases}
 			a_\pump + s(r-r_0)		& \text{for } r-r_0 < 0 \\
 			a_\pump e^{-2\alpha_\gamma(r-r_0)}	& \text{for } r-r_0 \geq 0
 		\end{cases},
\end{equation*}
with the unperturbed linewidth $\gamma_0$, decay coefficient $\alpha_\gamma$, amplitude of the exponential decay $a_\pump$, linear slope of the plateau at the resonator surface $s$, and the coordinate system offset $r_0$ as free parameters.

The relative backscattering amplitude grid was subsequently fitted with the parameters $\beta$ and $r_0$ fixed to the values obtained from the linewidth fit. Only the portion of data outside the resonator boundary, $r-r_0 = R \geq 0$, was fitted. The function fitted for the backscattering amplitude $A_\bs$ is derived in the Supplementary information, and reads
\begin{equation*}
	A_\bs(R,\phi)
	 = 
		\begin{cases}
			\text{not fitted}		& \text{for } R < 0 \\
 			|g|^2/\gamma^4(r, \phi) 	& \text{for } R \geq 0
 		\end{cases},
\end{equation*}
where $\gamma(r,\phi)$ is the fitted linewidth function, and the coupling from the forward- to the back-propagating mode
\begin{equation*}
	|g|^2 = g_0^2 + 2g_0a_\text{t}\,e^{-2\alpha_\bs R}\cos(\Theta) + a_\text{t}^2\,e^{-4\alpha_\bs R},
\end{equation*}
where $\gamma(r,\phi)$ is the fitted linewidth function, $g_0$ the intrinsic backscattering strength, $\Theta = k_\text{fr}\phi+\theta+\theta_R R$ is a position-dependent phase responsible for the fringe pattern, in which $\theta_R$ is a radially dependent phase accounting for the shape of the tip and/or drift. The period $\Delta$ of the fringe pattern is given by $k_\text{fr}=2\pi/\Delta$.

In order to sample arbitrary lines in the two-dimensional grid of measurement data shown in \creflett{fig:firstmment}{c--e} and \creflett{fig:secondmment}{b--c}, the grid data was interpolated linearly.


